F-Bench: Rethinking Human Preference Evaluation Metrics for Benchmarking Face Generation, Customization, and Restoration

Artificial intelligence generative models exhibit remarkable capabilities in content creation, particularly in face image generation, customization, and restoration. However, current AI-generated faces (AIGFs) often fall short of human preferences due to unique distortions, unrealistic details, and unexpected identity shifts, underscoring the need for a comprehensive quality evaluation framework for AIGFs. To address this need, we introduce FaceQ, a large-scale, comprehensive database of AI-generated Face images with fine-grained Quality annotations reflecting human preferences. The FaceQ database comprises 12,255 images generated by 29 models across three tasks: (1) face generation, (2) face customization, and (3) face restoration. It includes 32,742 mean opinion scores (MOSs) from 180 annotators, assessed across multiple dimensions: quality, authenticity, identity (ID) fidelity, and text-image correspondence. Using the FaceQ database, we establish F-Bench, a benchmark for comparing and evaluating face generation, customization, and restoration models, highlighting strengths and weaknesses across various prompts and evaluation dimensions. Additionally, we assess the performance of existing image quality assessment (IQA), face quality assessment (FQA), AI-generated content image quality assessment (AIGCIQA), and preference evaluation metrics, manifesting that these standard metrics are relatively ineffective in evaluating authenticity, ID fidelity, and text-image correspondence. The FaceQ database will be publicly available upon publication.

==> sec/tables/table3.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{ll}
    \toprule
        \multicolumn{2}{c}{Evaluation IDs}\\
    \midrule
   \Circled{1} Alan Turing
 &\Circled{14} Kamala Harris\\
\Circled{2} Albert Einstein &\Circled{15} Marilyn Monroe\\
      \Circled{3}  Anne Hathaway &\Circled{16} Mark Zuckerberg\\
\Circled{4} Audrey Hepburn &\Circled{17} Michelle Obama\\
        \Circled{5} Barack Obama&\Circled{18} Oprah Winfrey\\
\Circled{6} Bill Gates&\Circled{19} Renée Zellweger\\
\Circled{7} Donald Trump&\Circled{20} Scarlett Johansson\\
        \Circled{8} Dwayne Johnson&\Circled{21} Taylor Swift\\
\Circled{9} Elon Musk&\Circled{22} Thomas Edison\\
\Circled{10} Fei-Fei Li&\Circled{23} Vladimir Putin\\
\Circled{11} Geoffrey Hinton&\Circled{24} Woody Allen\\
\Circled{12} Jeff Bezos&\Circled{25} Yann LeCun\\
        \Circled{13} Joe Biden&\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{ID names used for evaluation.}}
    \label{tab:evaluate_ids}
\end{table}
